Multiple criteria hierarchy process for sorting problems under uncertainty applied to the evaluation of the operational maturity of research institutions

Despite the availability of qualified research personnel, up-to-date research facilities and experience in developing applied research and innovation, many worldwide research institutions face difficulties when managing contracted Research and Development (R&D) projects due to expectations from Industry (private sector). Such difficulties have motivated funding agents to create evaluation processes to check whether the operational procedures of funded research institutions are sufficient to provide timely answers to demand for innovation from industry and also to identify aspects that require quality improvement in research development. For this purpose, several multiple criteria decision-making approaches can be applied. Among the available multiple criteria approaches, sorting methods are one prominent tool to evaluate the operational capacity. However, the first difficulty in applying multiple criteria sorting methods is the need to hierarchically structure multiple criteria in order to represent the intended decision process. Additional challenges include the elicitation of the preference information and the definition of criteria evaluation, since these are frequently affected by some imprecision. In this paper, a new sorting method is proposed to deal with all of those critical points simultaneously. To consider multiple levels for the decision criteria, the FlowSort method is extended to account for hierarchical criteria. To deal with imprecise data, the FlowSort is integrated with fuzzy approaches. To yield solutions that consider fluctuations from imprecise weights, the Stochastic Multicriteria Acceptability Analysis is used. Finally, the proposed method is applied to the evaluation of research institutions, classifying them according to their operational maturity for development of applied research.

==> Apendice.tex <==
    Let $G_{1_1}$ and $G_{2_1}$ be macro-criteria ($f=2$) with weights $w_{1_1}=0.3$ e $w_{2_1}=0.7$, respectively. Each of macro-criteria has two sub-criteria of second level. As there are only 2 levels of criteria, these are also the elementary criteria. The sub-criteria of $G_{1_1}$ are denoted by $g_{1_1, 1}$ e $g_{1_1, 2}$ and the sub-criteria of $G_{2_1}$ are denoted by $g_{2_1, 1}$ e $g_{2_1, 2}$. We consider that the criteria $g_{1_1, 1}, g_{2_1, 1}$ and $g_{2_1, 2}$ shall be maximized and $g_{1_1, 2}$ minimized.
        
    In this decision problem, two alternatives, $x_1$ and $x_2$, should be assigned to two categories $C_1$ and $C_2$. Table \ref{tab: evaluation_example_flowsort_h} displays the performance values of the two alternatives seconds the elementary criteria. Table \ref{tab: profile_example_flowsort_h} presents the values of the limiting reference profiles that characterize the categories $C_1$ and $C_2$, also defined at the level of the elementary criteria.

         \begin{table}[h!]
            \centering
             \caption{Valores de desempenho das alternativas para cada um dos critérios elementares no exemplo numérico do método FlowSort-H.}
                \label{tab:avaliacao_exemplo_flowsort_h}
                \begin{tabular}{ccccc} \hline
                Alternativas	    &	$g_{1_1, 1}$	&	$g_{1_1, 2}$ & $g_{2_1, 1}$	&	$g_{2_1, 2}$   \\\hline
                $x_1$	            &	8	&	1	&	16	&	28	\\
                $x_2$	            &	9	&	3	&	8	&	12	\\\hline
            \end{tabular}
        \end{table}
        
        \begin{table}[h!]
            \centering
             \caption{Perfis de referência limitantes para cada um dos critérios elementares no exemplo numérico do método FlowSort-H.}
                \label{tab:perfil_exemplo_flowsort_h}
                \begin{tabular}{ccccc} \hline
                Perfis de referência	    &	$g_{1_1, 1}$	&	$g_{1_1, 2}$ & $g_{2_1, 1}$	&	$g_{2_1, 2}$   \\\hline
                $r_1$	            &	10	&	0	&	20	&	30	\\
                $r_2$	            &	5	&	5	&	10	&	15	\\
                $r_3$	            &	0	&	10	&	0	&	0	\\\hline
            \end{tabular}
        \end{table}
        
        In the FlowSort-H method, weights for the criteria of all levels must be defined such that the sum of the weights in a branch of the tree is not greater than 1. Thus, to the criteria $g_{1_1, 1}$ and $g_{1_1, 2}$ are assigned the weights $w_{1_1, 1}=0.2$ and $w_{1_1, 2}=0.8$, respectively. The criteria $g_{2_1, 1}$ and $g_{2_1, 2}$ are defined as the weights $w_{2_1, 1} = 0.4$ and $w_{2_1, 2}=0.6$. The weight of the criterion $G_{1_1}$ is $w_{1_1} = 0.3$ and the weight of criterion $G_{2_1}$ is $w_{2_1} = 0.7$. 

        To use the assignment rule \ref{net_attribute} (page 42), you must calculate the positive and negative flows of the alternatives and, for each alternative, the positive and negative flows of the reference profiles.
        
        The positive flow of the alternative $ x_1 $ is given by
            $$\phi^{+} (x_1) = \frac{1}{|R_i^{\mathbf{t}}| - 1} \sum_{y \in R_1-\{x_1\}} \pi(x_1, y),$$
        \noindent in which $R_1= R \cup \{x_1\} = \{r_1, r_2, r_3, x_1\}$ and, then, $|R_1| = 4$. Therefore, 
            $$\phi^{+} (x_1) = \frac{1}{3} [\pi(x_1, r_1) + \pi(x_1, r_2) + \pi(x_1, r_3)].$$
        Therefore, it is necessary to calculate the degrees of preference. To exemplify the calculation process, the calculation of 
        $\phi + (x_1, r_1)$ is given. Initially, it is necessary to calculate the preferences functions. The preference function of type 1 of Quadro was chosen \ref{tab: preferences_functions} (page 29). Thus, we have

        \begin{eqnarray*}
            P(g_{1_1, 1}(x_1), r_1) &=& P(d(g_{1_1, 1}(x_1) - r_1)) = P(8-10) = 0\\
            P(g_{1_1, 1}(x_1), r_2) &=& P(d(g_{1_1, 1}(x_1) - r_2)) = P(8-5) = 1\\
            P(g_{1_1, 1}(x_1), r_3) &=& P(d(g_{1_1, 1}(x_1) - r_3)) = P(8-0) = 1.
        \end{eqnarray*}
        Analogously, it is calculated the preference functions of the criteria $g_{2_1, 1}$ e $g_{2_1, 2}$. Como $g_{1_1, 2}$ should be minimized, one has to
        \begin{eqnarray*}
            P(g_{1_1, 2}(x_1), r_1) &=& P(d(r_1 - g_{1_1, 2}(x_1))) = P(0-1) = 0\\
            P(g_{1_1, 2}(x_1), r_2) &=& P(d(r_2) - g_{1_1, 2}(x_1)) = P(5-1) = 1\\
            P(g_{1_1, 2}(x_1), r_3) &=& P(d(r_3) - g_{1_1, 2}(x_1)) = P(10-1) = 1.
        \end{eqnarray*}
        The degrees of preference are then given by:
        \begin{eqnarray*}
            \pi(x_1, r_1) &=& w_{1_1}[w_{1_1, 1} P(g_{1_1, 1}(x_1), r_1)+ w_{1_1, 2} P(g_{1_1, 2}(x_1), r_1)]  \\
                          &+& w_{2_1}[w_{2_1, 1} P(g_{2_1, 1}(x_1), r_1)+ w_{2_1, 2} P(g_{2_1, 2}(x_1), r_1)] \\
                          &=& 0.3(0.2 * 0 + 0.8 * 0) + 0.7(0.4 *0 + 0.6* 0) = 0\\
            \pi(x_1, r_2) &=& 0.3(0.2 * 1 + 0.8 * 1) + 0.7(0.4 *1 + 0.6* 1) = 1\\
            \pi(x_1, r_3) &=& 0.3(0.2 * 1 + 0.8 * 1) + 0.7(0.4 *1 + 0.6* 1) = 1.
        \end{eqnarray*}
        Therefore, the positive flow of the alternative $ x_1 $ is given by
        $$\phi^{+}(R_1) = \frac{1}{3}(0+1+1) = \frac{2}{3} = 0.667.$$
        In an analogous way, the positive flows of the profiles related to the alternative $x_1$: $\phi^{+}_{R_1}(r_1)=1$, $\phi^{+}_{x_1}(r_2)=0.333$ e $\phi^{+}_{x_1}(r_3)=0$. Therefore, 
        $\phi^{+}_{R_1}(r_1) > \phi^{+}(x_1) > \phi^{+}_{x_1}(r_2)$. That is, the flow of the alternative $x_1$ is among the flows of the profiles that forms the category $C_1$. Thus, given the \ref{attribute_pos_flow} assignment rule (page 42), the alternative $x_1$ must be assigned to the $C_1$ category.
        
        Following the same calculation line, we obtain the positive, negative and total flows of the alternatives $x_1$ and $x_2$ and of the reference profiles, presented in Tables \ref{tab: flow_alte_hier} and \ref{tab: flow_profil_hier}, respectively.
        
        \begin{table}[h!]
            \small
            \centering
             \caption{Fluxos das alternativas no exemplo numérico do método FlowSort-H.}
                \label{tab:fluxo_alte_hier}
                \begin{tabular}{cccc} \hline
                Alternativas    &	$\phi^{+}(.)$	& $\phi^{-}(.)$ & $\phi(.)$ \\\hline
                 $x_1$          &	0.667	      &	0.333      &     0.333  	\\
                 $x_2$          &	0.433         &	0.566     &     -0.133 	\\\hline
            \end{tabular}
        \end{table}
        
        \begin{table}[h!]
            \small
            \centering
             \caption{Fluxos dos perfis limitantes no exemplo numérico do método FlowSort-H.}
                \label{tab:fluxo_perfil_hier}
                \begin{tabular}{ccccccc} \hline
                Alternativas    &	$\phi^{+}_{R_1}(.)$	& $\phi^{-}_{R_1}(.)$ & $\phi_{R_1}(.)$ &	$\phi^{+}_{R_2}(.)$	& $\phi^{-}_{R_2}(.)$ & $\phi_{R_2}(.)$\\\hline
                 $r_1$          &	1	            &	0        	&     1  	 & 1         &  0     & 1 \\
                 $r_2$          &	0.333	        &	0.666       &    -0.333  & 0.566	 & 0.433  &  0.133\\
                 $r_3$          &	0	            &	1        	&     -1 	 &  0        &   1    & -1	\\\hline
            \end{tabular}
        \end{table}
        
        Following the assignment rules defined in \ref{attribute_pos_flow}, \ref{assignment_neg_flow} and \ref{net_name assignment}, one has:

        \begin{eqnarray*}
           &\mbox{ Como }& \phi^{+}_{R_1} (r_1) = 1 \geqslant  \phi^{+} (x_1) = 0.667 > \phi^{+}_{R_1} (r_{2}) = 0.333, \mbox{ então } C_{\phi^{+}}(x_1) = C_1;\\
           &\mbox{ Como }& \phi^{-}_{R_1} (r_1) = 0 < \phi^{-}(x_1) = 0.333 \leqslant \phi^{-}_{R_1} (r_{2}) = 0.666, \mbox{ então } C_{\phi^{-}}(x_1) = C_1;\\
           &\mbox{ Como }& \phi_{R_1} (r_1) = 1 \geqslant \phi (x_1) =0.334 > \phi_{R_1} (r_2) = -0.333, \mbox{ então } C_{\phi}(x_1) = C_1.
        \end{eqnarray*}
        
        Thus, using any of the assignment rules, we have that the alternative $x_1$ is assigned to the category $C_1$. In the same way, it is concluded that, by applying any of the allocation rules, the alternative $x_2$ is assigned to the category $C_2$.
        
        To know in which of the criteria the alternative $x_2$ must improve to be assigned the category $C_1$, one must calculate the uni-criteria flows related to category $x_2$:
        
        \begin{eqnarray*}
            \phi_{g_{1_1}}^{+}(x_2) &=& \frac{1}{|R_2| - 1} \left(\sum_{h=1}^{3} \pi_{g_{1_1, 1}}(x_2, r_h) +\sum_{h=1}^{3} \pi_{g_{1_1, 2}}(x_2, r_h)\right)\\
                                    &=& \frac{1}{3} ((\pi_{g_{1_1, 1}}(x_2, r_1) + \pi_{g_{1_1, 1}}(x_2, r_2) + \pi_{g_{1_1, 1}}(x_2, r_3)) \\
                                    &~& + ~ (\pi_{g_{1_1, 2}}(x_2, r_1) + \pi_{g_{1_1, 2}}(x_2, r_2) + \pi_{g_{1_1, 2}}(x_2, r_3)))\\
                                    &=& \frac{1}{3}~ (w_{1_1, 1}(~P(d(g_{1_1, 1}(x_2) - r_1)) + P(d(g_{1_1, 1}(x_2) - r_2)) + P(d(g_{1_1, 1}(x_2) - r_3))) \\
                                    &~& + ~ w_{1_1, 2}(~P(d(g_{1_1, 2}(x_2) - r_1)) + P(d(g_{1_1, 2}(x_2) - r_2)) + P(d(g_{1_1, 2}(x_2) - r_3))))\\
                                    &=& \frac{1}{3}~ (0.2(0 + 1 + 1) + 0.8(0 + 1 + 1))\\
                                    &=& \frac{1}{3}~ (0.2(2) + 0.8(2)) = 0.667
                                    
          \end{eqnarray*}     
          \begin{eqnarray*}
            \phi_{g_{2_1}}^{+}(x_2) &=& \frac{1}{|R_2| - 1} \left(\sum_{h=1}^{3} \pi_{g_{2_1, 1}}(x_2, r_h) +\sum_{h=1}^{3}\pi_{g_{2_1, 2}}(x_2, r_h)\right)\\
                                    &=& \frac{1}{3} ((\pi_{g_{2_1, 1}}(x_2, r_1) + \pi_{g_{2_1, 1}}(x_2, r_2) + \pi_{g_{2_1, 1}}(x_2, r_3)) \\
                                    &~& + ~ (\pi_{g_{2_1, 2}}(x_2, r_1) + \pi_{g_{2_1, 2}}(x_2, r_2) + \pi_{g_{2_1, 2}}(x_2, r_3)))\\
                                    &=& \frac{1}{3}~ (w_{2_1, 1}(~P(d(g_{2_1, 1}(x_2) - r_1)) + P(d(g_{2_1, 1}(x_2) - r_2)) + P(d(g_{2_1, 1}(x_2) - r_3))) \\
                                    &~& + ~ w_{2_1, 2}(~P(d(g_{2_1, 2}(x_2) - r_1)) + P(d(g_{2_1, 2}(x_2) - r_2)) + P(d(g_{2_1, 2}(x_2) - r_3))))\\
                                    &=& \frac{1}{3}~ (0.4(0 + 0 + 1) + 0.6(0 + 0 + 1))\\
                                    &=& \frac{1}{3}~ (0.4(1) + 0.6(1)) = 0.333\\
        \end{eqnarray*}
        
        Flow of the alternative $ x_2 $ in relation to the second level criteria (in this case, also elementary criteria).
        \begin{eqnarray*}
        \phi_{g_{1_1, 1}}^{+}(x_2) &=& \frac{1}{|R_2| - 1} \left(\sum_{h=1}^{3} \pi_{g_{1_1, 1}}(x_2, r_h)\right)\\
                                    &=& \frac{1}{3} (\pi_{g_{1_1, 1}}(x_2, r_1) + \pi_{g_{1_1, 1}}(x_2, r_2) + \pi_{g_{1_1, 1}}(x_2, r_3)) \\
                                    &=& \frac{1}{3}~( P(d(g_{1_1, 1}(x_2) - r_1)) + P(d(g_{1_1, 1}(x_2) - r_2)) + P(d(g_{1_1, 1}(x_2) - r_3))) \\
                                    &=& \frac{1}{3}~ (0 + 1 + 1) = 0.667\\
        \phi_{g_{1_1, 2}}^{+}(x_2) &=& \frac{1}{|R_2| - 1} \left(\sum_{h=1}^{3} \pi_{g_{1_1, 2}}(x_2, r_h)\right)\\
                                    &=& \frac{1}{3} (\pi_{g_{1_1, 2}}(x_2, r_1) + \pi_{g_{1_1, 2}}(x_2, r_2) + \pi_{g_{1_1, 2}}(x_2, r_3)) \\
                                    &=& \frac{1}{3}~( P(d(g_{1_1, 2}(x_2) - r_1)) + P(d(g_{1_1, 2}(x_2) - r_2)) + P(d(g_{1_1, 2}(x_2) - r_3))) \\
                                    &=& \frac{1}{3}~ (0 + 1 + 1) = 0.667\\
        \phi_{g_{2_1, 1}}^{+}(x_2) &=& \frac{1}{|R_2| - 1} \left(\sum_{h=1}^{3} \pi_{g_{2_1, 1}}(x_2, r_h)\right)\\
                                    &=& \frac{1}{3} (\pi_{g_{2_1, 1}}(x_2, r_1) + \pi_{g_{2_1, 1}}(x_2, r_2) + \pi_{g_{2_1, 1}}(x_2, r_3)) \\
                                    &=& \frac{1}{3}~( P(d(g_{1_2, 1}(x_2) - r_1)) + P(d(g_{1_2, 1}(x_2) - r_2)) + P(d(g_{1_2, 1}(x_2) - r_3))) \\
                                    &=& \frac{1}{3}~ (0 + 0 + 1) = 0.333\\
        \phi_{g_{2_1, 2}}^{+}(x_2) &=& \frac{1}{|R_2| - 1} \left(\sum_{h=1}^{3} \pi_{g_{2_1, 2}}(x_2, r_h)\right)\\
                                    &=& \frac{1}{3} (\pi_{g_{2_1, 2}}(x_2, r_1) + \pi_{g_{2_1, 2}}(x_2, r_2) + \pi_{g_{2_1, 2}}(x_2, r_3)) \\
                                    &=& \frac{1}{3}~( P(d(g_{2_1, 2}(x_2) - r_1)) + P(d(g_{2_1, 2}(x_2) - r_2)) + P(d(g_{2_1, 2}(x_2) - r_3))) \\
                                    &=& \frac{1}{3}~ (0 + 0 + 1) = 0.333\\
        \end{eqnarray*}
        
        The values of the uni-criteria flows of the alternative $x_2$ calculated above are shown in the Table \ref{tab: flux_alt_uni}. Following the same calculation line, the values of the uni-criteria flows of the reference profiles are obtained. The values are shown in the Table \ref{tab: perf_profile_uni}.

        
        \begin{table}[h!]
            \small
            \centering
             \caption{Fluxos uni-critérios da alternativa $x_2$ no exemplo numérico do método FlowSort-H.}
                \label{tab:fluxo_alt_uni}
                \begin{tabular}{ccccccc} \hline
                Alternativa    & $\phi_{g_{1_1}}(.)$ & $\phi_{g_{2_1}}(.)$ & $\phi_{g_{1_1, 1}}(.)$	& $\phi_{g_{1_1, 2}}(.)$ & $\phi_{g_{2_1, 1}}(.)$ & $\phi_{g_{2_1, 2}} (.)$ \\\hline
                 $x_2$          &  0.667     & 0.333   &    0.667   & 0.667  & 0.333 & 0.333\\\hline
            \end{tabular}
        \end{table}
    
        \begin{table}[h!]
            \small
            \centering
             \caption{Fluxos uni-critérios dos perfis limitantes no exemplo numérico do método FlowSort-H.}
                \label{tab:fluxo_perfis_uni}
                \begin{tabular}{ccccccc} \hline
                Alternativa/ Perfil    & $\phi_{R_2, g_{1_1}}(.)$ & $\phi_{R_2, g_{2_1}}(.)$ & $\phi_{R_2, g_{1_1, 1}}(.)$	& $\phi_{R_2, g_{1_1, 2}}(.)$ & $\phi_{R_2, g_{2_1, 1}}(.)$ & $\phi_{R_2, g_{2_1, 2}} (.)$ \\\hline
                 $x_2$          &  0.667     & 0.333   &    0.667   & 0.667  & 0.333 & 0.333\\\hline
                 $r_1$          &	1	      &	1      &     1      & 1      & 1     & 1  	\\
                 $r_2$          &	- 0.333	  &	0.333  &     -0.333 & -0.333 & 0.333 & 0.333  	\\
                 $r_3$          &	-1	      &	-1     &     -1    & -1      & -1    & -1   	\\\hline
            \end{tabular}
        \end{table}

       Thus, $\phi_{R_2, g_{1_1}}(r_1) &=& 1 \geqslant \phi (x_2) =0.667 > \phi_{R_2, g_{1_1}}(r_2) = - 0.333$. Therefore, $C_{\phi}(x_2) &=& C_1$ regarding criterion $g_{1_1}$. Analogously, $\phi_{R_2, g_{2_1}}(r_2) &=& 0.333 \geqslant \phi (x_2) =0.333 > \phi_{R_2, g_{2_1}}(r_3) = - 1$, and therefore $C_{\phi}(x_2) &=& C_2$ when the alternative $x_2$ is analyzed only regarding criterion $g_{2_1}$.
        
        Analyzing the sub-criteria of the criterion $g_{2_1}$, we have $C_{\phi}(x_2) = C_2$ for both the criteria $g_{2_1, 1}$ and $g_{2_1, 2}$. Therefore, improving the performances of the alternative $x_2$ regarding criteria $g_{2_1, 1}$ and $g_{2_1, 2}$ shall result, at some point of this improvement, in an assignment of the alternative $x_2$ to category $C_1$.
